Accelerating Diffusion Sampling via Exploiting Local Transition Coherence

Text-based diffusion models have made significant breakthroughs in generating high-quality images and videos from textual descriptions. However, the lengthy sampling time of the denoising process remains a significant bottleneck in practical applications. Previous methods either ignore the statistical relationships between adjacent steps or rely on attention or feature similarity between them, which often only works with specific network structures. To address this issue, we discover a new statistical relationship in the transition operator between adjacent steps, focusing on the relationship of the outputs from the network. This relationship does not impose any requirements on the network structure. Based on this observation, we propose a novel training-free acceleration method called LTC-Accel, which uses the identified relationship to estimate the current transition operator based on adjacent steps. Due to no specific assumptions regarding the network structure, LTC-Accel is applicable to almost all diffusion-based methods and orthogonal to almost all existing acceleration techniques, making it easy to combine with them. Experimental results demonstrate that LTC-Accel significantly speeds up sampling in text-to-image and text-to-video synthesis while maintaining competitive sample quality. Specifically, LTC-Accel achieves a speedup of 1.67-fold in Stable Diffusion v2 and a speedup of 1.55-fold in video generation models. When combined with distillation models, LTC-Accel achieves a remarkable 10-fold speedup in video generation, allowing real-time generation of more than 16FPS.

==> rebuttal_sec/00_heading.tex <==


% We would like to thank all the reviewers for your constructive feedback on our paper.
% We appreciate the recognition of the novelty (\reviewerA{A}), generalizability (\reviewerB{B}) and effectiveness (\reviewerC{C}), as well as the insightful suggestions that have helped us improve our work.
% Below, we provide detailed responses to each comment.
We sincerely thank the reviewers for their constructive feedback and positive recognition. In particular, we appreciate the comments that our motivation is clear, the method is novel and theoretically grounded, orthogonal to existing acceleration techniques, and the experiments are thorough and robust (\reviewerA{A}, \reviewerB{B}, \reviewerC{C}). We first address several common concerns raised across the reviews, followed by point-by-point responses to each reviewer.

==> rebuttal_sec/fig_exp.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \begin{tikzpicture}[scale=0.5]
        \begin{axis}[
            xlabel={Step},
            ylabel={Metric},
            % x dir=reverse,
            xlabel style={xshift=3pt},
            ylabel style={yshift=-5pt, xshift=2pt},
            xmin=10, xmax=45,
            % ymin=0.3,
            % ymin=0.4, ymax=1.1,
            xtick={20,30,40},
            ytick = {0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
            % ytick={0.5,0.6,...,1.0},
            % y tick label style={
            %     /pgf/number format/.cd, 
            %     fixed,
            %     precision=1,
            %     zerofill,
            % },
            grid=major,
            grid style={gray!30, loosely dashed}, % 更优雅的网格线
            legend style={at={(0.35,0.8)}, anchor=north, font=\small, draw=none, fill=white, fill opacity=0.8},
            axis line style={line width=1pt},
            tick style={line width=0.8pt},
            every axis plot/.append style={line width=1.2pt, smooth, line cap=round}
        ]
         
        \addplot[color=myorange!80!black,dash dot dot,dash phase=2pt,
        ] table[x=Step,y=Imaging_Quality,col sep=comma
        ]{Rebuttal_Fig_and_Data/video_org.csv};
        \addlegendentry{Org  (Imaging Quality)}

        \addplot[color=yellow!80!black, dash dot dot, dash phase=2pt] 
            table[x=Step, y=Temporal_Flickering, col sep=comma]{Rebuttal_Fig_and_Data/video_org.csv};
        \addlegendentry{Org (Temporal Flickering)}

        \addplot[color=myorange!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        mark options={solid, fill=myorange!90!black}] 
            table[x=Step, y=Imaging_Quality, col sep=comma]{Rebuttal_Fig_and_Data/video_ltc.csv};
        \addlegendentry{Ours (Imaging Quality)}

        \addplot[color=yellow!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        mark options={solid, fill=myorange!90!black}] 
            table[x=Step, y=Temporal_Flickering, col sep=comma]{Rebuttal_Fig_and_Data/video_ltc.csv};
        \addlegendentry{Ours (Temporal Flickering)}
    
        \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \captionsetup{justification=justified, singlelinecheck=true}
        \caption{\methodabbr on CogVideoX.}
        \label{fig:video_iq}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \begin{tikzpicture}[scale=0.5]
        \begin{axis}[
            % ybar,
            % bar width=8pt,
            % enlarge x limits=0.05, 
            % ybar=0.5pt, % 组间间距为0
            xlabel={Step},
            ylabel={ImageReward},
            % x dir=reverse,
            xlabel style={xshift=3pt},
            ylabel style={yshift=-8pt, xshift=8pt},
            xmin=5, xmax=35,
            % ymin=0.1,
            % ymin=0.352, ymax=0.385,
            xtick={10,20,30},
            % ytick={0.360,0.365,0.370,0.375,0.380},
            % yticklabel style={/pgf/number format/.cd, fixed, precision=3, zerofill}, 
            grid=major,
            grid style={gray!30, loosely dashed},
            legend style={at={(0.2,0.95)}, anchor=north, font=\small, draw=none, fill=white, fill opacity=0.8},
            axis line style={line width=1pt},
            tick style={line width=0.8pt},
            every axis plot/.append style={line width=1.2pt, smooth, line cap=round}
        ]

        \addplot[color=mygreen!80!black,dash dot dot,dash phase=2pt,] coordinates{(10,0.1332)(20,0.16318321711494355)(30,0.1901330420449376)};
        \addlegendentry{AYS}


        \addplot[color=mygreen!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        mark options={solid, fill=mygreen!90!black}] coordinates{(8,0.1309)(15,0.16936568364390406)(20,0.21305280066886917)};
        \addlegendentry{AYS+Ours}

        % \addplot[color=mygreen!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        % mark options={solid, fill=mygreen!90!black}] coordinates{(8,0.1309)(15,0.15096489753137576)(20,0.21305280066886917)};
        % \addlegendentry{AYS+Ours}

        

      
        % \addplot[color=myred!80!black] 
        %     table[x=Step, y=Guidance, col sep=comma]{section/Data/angle_and_guidance/guidance_mean.csv};
        % \addlegendentry{Guidance Scale}
    
        \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \captionsetup{justification=justified, singlelinecheck=true}
        \caption{AYS at 10, 20 and 30.}
        \label{fig:ays}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \begin{tikzpicture}[scale=0.5]
        \begin{axis}[
            ybar,
            bar width=6pt,
            xlabel={$\tau$ (Acceleration interval)},
            ylabel={ImageReward},
            % x dir=reverse,
            xlabel style={xshift=3pt},
            ylabel style={yshift=-5pt, xshift=2pt},
            xmin=-0.15, xmax=0.45,
            % ymin=0.4, ymax=1.1,
            xtick={0.15,0.2,0.25,0.4},
            % ytick={0.5,0.6,...,1.0},
            % y tick label style={
            %     /pgf/number format/.cd, 
            %     fixed,
            %     precision=1,
            %     zerofill,
            % },
            grid=major,
            grid style={gray!30, loosely dashed}, % 更优雅的网格线
            legend style={at={(0.2,0.95)}, anchor=north, font=\small, draw=none, fill=white, fill opacity=0.8},
            axis line style={line width=1pt},
            tick style={line width=0.8pt},
            every axis plot/.append style={line width=1.2pt, smooth, line cap=round}
        ]
         
        \addplot[ybar,draw=none,fill=Red0!95!black, bar shift=0pt] coordinates{(0.1,0.4131923627264332)};
        \addlegendentry{SD v2 Org}

        \addplot[ybar,draw=none,fill=Red1, bar shift=0pt] coordinates{(0.4,0.3352907943807077)};
        \addlegendentry{Interval [2,39]}

        \addplot[ybar,draw=none,fill=Red2, bar shift=0pt] coordinates{(0.25,0.3483917866908014)};
        \addlegendentry{Interval [6,39]}

        \addplot[ybar,draw=none,fill=Red3, bar shift=0pt] coordinates{(0.2,0.40142159098340197)};
        \addlegendentry{Interval [10,39]}

        \addplot[ybar,draw=none,fill=Red4, bar shift=0pt] coordinates{(0.15,0.4226344387261197)};
        \addlegendentry{Interval [14,39]}

        \addplot[color=mypurple!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        mark options={solid, fill=mypurple!90!black}] coordinates{(0.4,0.3352907943807077)(0.25,0.3483917866908014)(0.2,0.40142159098340197)
        (0.15,0.4226344387261197)};
        \addlegendentry{Variation}
    
        \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \captionsetup{justification=justified, singlelinecheck=true}
        \caption{$\tau$ selection at 40.}
        \label{fig:interval}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \begin{tikzpicture}[scale=0.5]
        \begin{axis}[
            ybar,
            bar width=6pt,
            % enlarge x limits=0.05, 
            ybar=0.5pt, % 组间间距为0
            xlabel={Step},
            ylabel={ImageReward},
            % x dir=reverse,
            xlabel style={xshift=3pt},
            ylabel style={yshift=-8pt, xshift=8pt},
            xmin=30, xmax=45,
            % ymin=0.1,
            % ymin=0.352, ymax=0.385,
            xtick={30,35,40},
            % ytick={0.360,0.365,0.370,0.375,0.380},
            % yticklabel style={/pgf/number format/.cd, fixed, precision=3, zerofill}, 
            grid=major,
            grid style={gray!30, loosely dashed},
            legend style={at={(0.3,0.95)}, anchor=north, font=\scriptsize, draw=none, fill=white, fill opacity=0.8},
            axis line style={line width=1pt},
            tick style={line width=0.8pt},
            every axis plot/.append style={line width=1.2pt, smooth, line cap=round}
        ]

        % \addplot[ybar,draw=none,fill=mygreen!60!white,bar shift=-3pt] coordinates{(20,0.16318321711494355)(30,0.1901330420449376)};
        % \addlegendentry{Ays}

        % \addplot[ybar,draw=none,fill=myblue!60!white,bar shift=3pt] coordinates{(20,0.15096489753137576)(30,0.21305280066886917)};
        % \addlegendentry{Ays+Ours}

        % \addplot[ybar,draw=none,fill=Red0!95!black, bar shift=-18pt] coordinates{(40,0.4131923627264332)};
        % \addlegendentry{SD v2 Org}

        \addplot[ybar,draw=none,fill=Blue1!50!white, bar shift=-10pt] coordinates{(40,0.3352907943807077)};
        \addlegendentry{Interval [2,39], Bias=0}

        % \addplot[ybar,draw=none,fill=Red2, bar shift=-6pt] coordinates{(40,0.3483917866908014)};
        % \addlegendentry{Interval [6,39]}

        % \addplot[ybar,draw=none,fill=Red3, bar shift=0pt] coordinates{(40,0.40142159098340197)};
        % \addlegendentry{Interval [10,39]}

        \addplot[ybar,draw=none,fill=Blue2, bar shift=-4pt] coordinates{(40,0.41347503241128286)};
        \addlegendentry{Interval [2,39], Bias=0.05}

        \addplot[ybar,draw=none,fill=Blue4, bar shift=4pt] coordinates{(40,0.4226344387261197)};
        \addlegendentry{Interval [14,39],$\phi=\sqrt{SNR(t)}$}
% $\phi=\sqrt{\alpha(t)/\beta(t)}$
        \addplot[ybar,draw=none,fill=Blue6, bar shift=10pt] coordinates{(40,0.40184151700540677)};
        \addlegendentry{Interval [14,39],$\phi'=SNR(t)$}

        % \addplot[ybar,draw=none,fill=Blue6, bar shift=9pt] coordinates{(40,0.41347503241128286)};
        % \addlegendentry{Interval [2,39], Bias=0.05}

      
        % \addplot[color=myred!80!black] 
        %     table[x=Step, y=Guidance, col sep=comma]{section/Data/angle_and_guidance/guidance_mean.csv};
        % \addlegendentry{Guidance Scale}
    
        \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \captionsetup{justification=justified, singlelinecheck=true}
        \caption{$\phi$ and bias at 40. }
        \label{fig:phi+bias}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Comparative experiments on video generations, compatibility with AYS, and ablation studies on interval selection, $\phi$ and bias.}
    \vspace{-22pt}
    \label{fig:re_exp}
    
\end{figure*}

==> rebuttal_sec/reviewer1-5.tex <==
\section{Performance of \methodabbr on DiT (\reviewerC{C}).}

We would like to kindly clarify that we have conducted experiments on Stable Diffusion v3.5 in Figure $5$c and $5$f, with visual results shown in Figure $1$.

\section{Integration with Distillation (\reviewerC{C}).}

We understand your concern on distillation, and our method can collaborate well with distillation techniques as presented in Table $4$ and Figure $2$b.

\section{Typos (\reviewerC{C}).}

We appreciate your careful review on our paper and we are pleased to accept your kind corrections. Thank you for your recognition and suggestions again!

==> sec/Fig_Tab_Code/fig_ays.tex <==
\begin{figure}[t]
        \begin{tikzpicture}[scale=0.9]
        \begin{axis}[
            % ybar,
            % bar width=8pt,
            % enlarge x limits=0.05, 
            % ybar=0.5pt, % 组间间距为0
            xlabel={Step},
            ylabel={ImageReward},
            % x dir=reverse,
            xlabel style={xshift=3pt},
            ylabel style={yshift=-8pt, xshift=8pt},
            xmin=5, xmax=35,
            % ymin=0.1,
            % ymin=0.352, ymax=0.385,
            xtick={10,20,30},
            % ytick={0.360,0.365,0.370,0.375,0.380},
            % yticklabel style={/pgf/number format/.cd, fixed, precision=3, zerofill}, 
            grid=major,
            grid style={gray!30, loosely dashed},
            legend style={at={(0.2,0.95)}, anchor=north, font=\small, draw=none, fill=white, fill opacity=0.8},
            axis line style={line width=1pt},
            tick style={line width=0.8pt},
            every axis plot/.append style={line width=1.2pt, smooth, line cap=round}
        ]

        \addplot[color=mygreen!80!black,dash dot dot,dash phase=2pt,] coordinates{(10,0.1332)(20,0.16318321711494355)(30,0.1901330420449376)};
        \addlegendentry{AYS}


        \addplot[color=mygreen!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        mark options={solid, fill=mygreen!90!black}] coordinates{(8,0.1309)(15,0.16936568364390406)(20,0.21305280066886917)};
        \addlegendentry{AYS+Ours}

        % \addplot[color=mygreen!80!black, line width=1.8pt, dash pattern=on 0pt off 0pt, mark=triangle*, 
        % mark options={solid, fill=mygreen!90!black}] coordinates{(8,0.1309)(15,0.15096489753137576)(20,0.21305280066886917)};
        % \addlegendentry{AYS+Ours}

        

      
        % \addplot[color=myred!80!black] 
        %     table[x=Step, y=Guidance, col sep=comma]{section/Data/angle_and_guidance/guidance_mean.csv};
        % \addlegendentry{Guidance Scale}
    
        \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \captionsetup{justification=justified, singlelinecheck=true}
        \caption{AYS at 10, 20 and 30.}
        \label{fig:ays_ltc}
    \end{figure}
